Channel Vision Transformers: An Image Is Worth 1 x 16 x 16 Words

Vision Transformer (ViT) has emerged as a powerful architecture in the realm of modern computer vision. However, its application in certain imaging fields, such as microscopy and satellite imaging, presents unique challenges. In these domains, images often contain multiple channels, each carrying semantically distinct and independent information. Furthermore, the model must demonstrate robustness to sparsity in input channels, as they may not be densely available during training or testing. In this paper, we propose a modification to the ViT architecture that enhances reasoning across the input channels and introduce Hierarchical Channel Sampling (HCS) as an additional regularization technique to ensure robustness when only partial channels are presented during test time. Our proposed model, ChannelViT, constructs patch tokens independently from each input channel and utilizes a learnable channel embedding that is added to the patch tokens, similar to positional embeddings. We evaluate the performance of ChannelViT on ImageNet, JUMP-CP (microscopy cell imaging), and So2Sat (satellite imaging). Our results show that ChannelViT outperforms ViT on classification tasks and generalizes well, even when a subset of input channels is used during testing. Across our experiments, HCS proves to be a powerful regularizer, independent of the architecture employed, suggesting itself as a straightforward technique for robust ViT training. Lastly, we find that ChannelViT generalizes effectively even when there is limited access to all channels during training, highlighting its potential for multi-channel imaging under real-world conditions with sparse sensors. Our code is available at https://github.com/insitro/ChannelViT.

==> sections/interpretability.tex <==
\section{Attention Visualization}
In addition to performance and generalization across variable channel lengths, we also evaluated the utility of ChannelViT for interpreting importance of visual features across channels using attention rollout mechanisms. For this, we used the methodology in \cite{chefer2021transformer} that integrates gradients and relevancy scores across layers of the transformer network. 


\begin{figure}[h]
     \begin{center}
    %\framebox[4.0in]{$\;$}
     \includegraphics[width=1.0\textwidth]{figures/imagenet_attention_rollout.png}
   \end{center}
    \caption{(a, c) Relevancy visualization on ViT architecture showing spatially resolved attention maps; (b,d) Relevancy visualization in Channel-ViT where we can observe attention maps factored by the input channel contributions on natural images}
     \label{fig:imagenet_rollout}
\end{figure}






